Emergent Geometry from Quantum Probability

Carrying the insights of conditional probability to the quantum realm is notoriously difficult due to the non-commutative nature of quantum observables. Nevertheless, conditional expectations on von Neumann algebras have played a significant role in the development of quantum information theory, and especially the study of quantum error correction. In quantum gravity, it has been suggested that conditional expectations may be used to implement the holographic map algebraically, with quantum error correction underlying the emergence of spacetime through the generalized entropy formula. However, the requirements for exact error correction are almost certainly too strong for realistic theories of quantum gravity. In this note, we present a relaxed notion of quantum conditional expectation which implements approximate error correction. We introduce a generalization of Connes' spatial theory adapted to completely positive maps, and derive a chain rule allowing for the non-commutative factorization of relative modular operators into a marginal and conditional part, constituting a quantum Bayes' law. This allows for an exact quantification of the information gap occurring in the data processing inequality for arbitrary quantum channels. When applied to algebraic inclusions, this also provides an approach to factorizing the entropy of states into a sum of terms which, in the gravitational context, may be interpreted as a generalized entropy. We illustrate that the emergent area operator is fully non-commutative rather than central, except under the conditions of exact error correction. We provide some comments on how this result may be used to construct a fully algebraic quantum extremal surface prescription and to probe the quantum nature of black holes.

==> LeighMacro.tex <==
% last update: RGL 2022-12-15
% special macro file for research note (see template note_template.tex)

\input{packages.tex}
\input{standard.tex}
\usepackage{mdframed,framed}

% set up sans serif fonts in text and in mathmode
\renewcommand{\familydefault}{\sfdefault}
\usepackage{sfmath}

% generic pages setups
\textwidth = 7 in
\textheight = 9.0 in
\oddsidemargin = -0.25 in
\evensidemargin = -0.25 in
\topmargin = -0.5 in
\headheight = 0.0 in
\headsep = 0.0 in
\parskip = 0.2in
\parindent = 0.2in
%
%\newcommand{\comment}[1]{}
\newcommand{\mf}{\mathfrak{}}

\newcommand{\margnote}[1]{\marginpar{#1}}

\setlength\cftparskip{-1pt}
\setlength\cftbeforesecskip{5pt}
\setlength\cftaftertoctitleskip{2pt}

% Boxes
\def\mybox#1{\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{#1}}}
\def\mytbox#1#2{\noindent
	\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{{\bf #1}}}\\ 
	\framebox[\textwidth]{\parbox[t]{0.95\textwidth}{#2}}
	}

% shaded quote box
\mdfdefinestyle{MyShadeQuoteStyle}{%
    leftmargin=15pt,
    rightmargin=15pt,
    backgroundcolor=gray!25,
    linewidth=0pt,
    skipbelow=\topskip,
    skipabove=\topskip
	}


\newenvironment{shadequote}[1][]{%
    \ignorespaces%
    \begin{mdframed}[style=MyShadeQuoteStyle,#1]%
	}{%
    \end{mdframed}%
    \ignorespacesafterend%
	}%

\newenvironment{wideshadequote}%
{\begin{snugshade}\begin{quote}}
{\hfill\end{quote}\end{snugshade}}

\definecolor{shadecolor}{rgb}{0.9,0.9,0.9}

% the title box for notes
\newlength{\leftfield}          \setlength{\leftfield}{1.5in}
\newlength{\centerfield}        \setlength{\centerfield}{3.4in}
\newlength{\rightfield}         \setlength{\rightfield}{1.9in}
								\setlength{\fboxrule}{1px}
								
\newcommand{\twodigits}[1]{\ifnum#1<10 0\fi\number#1}
	
\newcommand{\mytitlebox}[4]{
	\framebox[\textwidth]{
	\begin{minipage}[c]{\textwidth}
		\makebox[\leftfield][l]{\littlefig{Physics-logo-small.png}{3} 
		%\littlefig{PI_logo.png}{1.3}
		}\ 
		\begin{minipage}[b]{\centerfield}
			\begin{center}{\bf\large #1}\\ #2\end{center}
		\end{minipage} 
		\begin{minipage}[b]{\rightfield}
			\begin{flushright}
				#3\\ Create: #4\\ Update: \the\year--\twodigits\month--\twodigits\day 
			\end{flushright}
		\end{minipage} 
	\end{minipage}
	}
}	

\setlength{\headsep}{4 ex}
\pagestyle{myheadings}
\markright{\title\ (\author)}

%\RequirePackage{color}

% display references as hyperlinks
\newcommand{\displayref}[2]{\href[pdfnewwindow]{#1}{{\color{BrickRed}[#2]}}}

\newcounter{example}
\setcounter{example}{0}
\renewcommand{\theexample}{\arabic{section}.\arabic{example}}
\newcommand*\examplelabel[1]{\hspace\labelsep\normalfont\bfseries #1}
\newenvironment{example}[1]{\refstepcounter{example}\label{exmpl:#1}\let\makelabel\examplelabel
    \begin{mdframed}[
       frametitle={{\bf Example \theexample: #1}},
       frametitlerule=true,
       frametitlebackgroundcolor=black!20,
       frametitlebelowskip=0.5\topskip,
       outerlinewidth = 1,
       roundcorner = 5pt,
       leftmargin=20pt,
       rightmargin=20pt,
       innerleftmargin=10pt,
       innerlinewidth=1.0pt,
       innertopmargin=0.5\topskip
    ]
}{
    \end{mdframed}
}

